A Heuristically Assisted Deep Reinforcement Learning Approach for Network Slice Placement

Network Slice placement with the problem of allocation of resources from a virtualized substrate network is an optimization problem which can be formulated as a multiobjective Integer Linear Programming (ILP) problem. However, to cope with the complexity of such a continuous task and seeking for optimality and automation, the use of Machine Learning (ML) techniques appear as a promising approach. We introduce a hybrid placement solution based on Deep Reinforcement Learning (DRL) and a dedicated optimization heuristic based on the Power of Two Choices principle. The DRL algorithm uses the so-called Asynchronous Advantage Actor Critic (A3C) algorithm for fast learning, and Graph Convolutional Networks (GCN) to automate feature extraction from the physical substrate network. The proposed Heuristically-Assisted DRL (HA-DRL) allows to accelerate the learning process and gain in resource usage when compared against other state-of-the-art approaches as the evaluation results evidence.

==> Backup/Background.tex <==
\subsection{Reinforcement Learning (RL) Background\label{sec:rlbackground}}
% Reinforcement learning part
\renewcommand{\sset}{\Sigma}
%According to \cite{sutton2018reinforcement}, Reinforcement Learning (RL) is simultaneously a class of problems, a class of solution methods that work well on these problems, and the field that studies these problems together with their solution methods. The question in RL problems is how to learn from interaction to achieve a goal. 

The standard RL setup comprises a Agent that interacts with what is called Environment at each step of a discrete time series $t = 0,1,2,3..., T$. At each time step the agent receives some representation of the Environment's state $\sigma_t \in \Sigma$, where $\Sigma$ is the set of possible states, and selects some Action $a_t \in \aset$ to perform, where $\aset$ is the set of possible actions. The action performed by the Agent modifies its Environment accordingly, leads  to a new State $\sigma_{t+1}$ of the Agent, and generates a Reward $r_{t+1} \in \mathbb{R}$. 

The Reward is a special numerical value that formalizes the Agent's goal. In general, the agent tries to maximize the sum of discounted Rewards. This objective is called Return and can be formalized as $G_t = \sum^{T-t-1}_{k=0}\gamma^{k} r_{t+k+1}$ \cite{sutton2018reinforcement}.

To select the Action to perform, the Agent relies on a Policy $\pi: \sset \times \aset \rightarrow \mathbb{R}$ that maps each Action $a \in \aset$ and State $\sigma \in \sset$ to the probability $\pi(a,\sigma)$ of taking Action $a$ in State $\sigma$. 

For a specific Policy, we can define the concept of State-value function $$v_{\pi}(t;\sigma)=\mathbb{E}_{\pi}\left[\sum^{T-t-1}_{k=0}\gamma^{k} r_{t+k+1} | \sigma_t = \sigma \right]$$
%\textbf{Cette quantite depend de t !} \textbf{J:j'ai inséré t comme un paramêtre}
as the expected return when starting on state $\sigma$ and following Policy $\pi$ thereafter. An interesting property is defined from State-value functions since they allow the definition of a partial order between policies: $\pi \geq \pi'$ if and only if $v_{\pi}(\sigma) \geq v_{\pi'}(\sigma)$ $\forall \sigma \in \sset$. 

As a corollary there is always at least one policy $\pi^*$ that is better than or equal to all other policies. This Policy is called the optimal Policy and it is associated with an optimal State-value function $v_{\pi^*}$\cite{sutton2018reinforcement}. However, differently from Optimal Control Theory, RL agents can only access the system transition probabilities (i.e., $p(\sigma'|\sigma,a)$) trough sampling. Hence, $\pi^*$ and $v_{\pi^*}$ can only be accessed by approximation \cite{sutton2018reinforcement}.
 
 \subsection{Deep Reinforcement Learning (DRL) Background }
% Deep Reinforcement Learning
Deep Reinforcement Learning (DRL) refers to the usage of Deep Learning to improve the function approximation needed to solve RL problems. DRL frameworks often represent the Policy and other learned functions (i.e., State-value function) as Deep Neural Networks and develop specialized algorithms that perform well in this setting. 

As usual with neural networks, a Loss function $J(\theta)$ is defined to measure the error between the estimated functions and appropriate target values. Typically, a minimum of this loss function is computed using some iterative optimization algorithm (i.e., gradient descent) based on the gradients $\nabla J(\theta)$.



==> Backup/SOTA_heuristics.tex <==
\subsection{On heuristics for slice placement optimization \label{sec:on_heuristics}}

Most of the works on network slice placement optimization propose heuristic approaches to addressing the scalability issues due to the ever-growing complexity of exact approaches like ILP (see \cite{cnsm_2020} for an extensive list of heuristics for slice placement). Most of existing heuristics are static and use centralized strategies, mostly online algorithms,  where placement requests arrive dynamically and  are not known in advance as opposed to offline  algorithms. However even efficient heuristic approaches present some drawbacks: i) they have difficulties to handle multiple optimization criteria, ii) they are not scalable enough real online placement scenarios, and iii) they are not flexible enough due to manual design of features used to solve the problem. We focus then on ML based approaches as they are seen as potential solutions for these problems.



==> Backup/SOTA_tables.tex <==
\begin{table*}
\centering
\caption{Deep Reinforcement Learning Modeling and Training Strategies}
\label{table4}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Reference}}                   & \multicolumn{2}{c}{\textbf{Convolutional Layers Used}} & \multicolumn{2}{c}{\textbf{Training Algorithm}} \\ \cmidrule(l){2-5} 
                                                      & GCN                        & CNN                       & Value Based            & Policy-based           \\ \midrule
\cite{p1}                 & \checkmark                          &                           &                        & A3C                    \\ \midrule
\cite{rkhami2021learn} & \checkmark                          &                           &                        & REINFORCE              \\ \midrule
\cite{p2}              &                            & \checkmark                         & Deep Q-Learning        &                        \\ \midrule
\cite{p3}               &                            & \checkmark                         &                        & RMSProp                \\ \midrule
\cite{p4}               &                            & \checkmark                         &                        & Policy Gradient        \\ \midrule
\cite{p5}                &                            &                           &                        & Policy Gradient        \\ \midrule
\cite{p8,quang2019deep}                &                            & \checkmark                         &                        & DDPG                   \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Deep Reinforcement Learning Framework Components and Network Scale}
\label{table5}
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Reference}} &
  \multicolumn{4}{c}{\textbf{State Features}} &
  \multicolumn{4}{c}{\textbf{Reward Function}} &
  \multicolumn{2}{c}{\textbf{Network Scale}} \\ \cmidrule(l){2-11} 
 &
  CPU &
  Memory &
  Bandwith &
  Latency &
  \begin{tabular}[c]{@{}c@{}}Acceptance \\ Ratio\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Load \\ Balance\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Cost and \\ Revenue\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}SLA \\ Satisfaction\end{tabular} &
  Small &
  Medium \\ \midrule
\cite{p1}                 & \checkmark &   & \checkmark &   & \checkmark & \checkmark & \checkmark &   &   & \checkmark \\ \midrule
\cite{rkhami2021learn} & \checkmark &   & \checkmark &   &   &   & \checkmark &   &   & \checkmark \\ \midrule
\cite{p2}              & \checkmark &   & \checkmark &   &   &   & \checkmark &   & \checkmark &   \\ \midrule
\cite{p3}                & \checkmark & \checkmark & \checkmark & \checkmark &   &   &   & \checkmark & \checkmark &   \\ \midrule
\cite{p4}                & \checkmark &   & \checkmark & \checkmark & \checkmark &   & \checkmark &   &   & \checkmark \\ \midrule
\cite{p5}                & \checkmark &   & \checkmark &   &   &   & \checkmark &   &   & \checkmark \\ \midrule
\cite{quang2019deep}    & \checkmark &   & \checkmark & \checkmark & \checkmark &   &   &   &   & \checkmark \\ \midrule
\cite{p8}               & \checkmark &   & \checkmark & \checkmark &   &   & \checkmark &   &   & \checkmark \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Summary of Recent Works on Deep Reinforcement Learning for Network Slice Placement}
\label{tab:SOTA_1}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Reference}} &
  \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}State \\ Features\end{tabular}}} &
  \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Reward \\ Function\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Use of \\ Convolutions\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Algorithm\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Use of\\ Heuristics\end{tabular}}} \\ \cmidrule(lr){2-13}
 &
  CPU &
  Storage &
  Bandwith &
  Latency &
  \begin{tabular}[c]{@{}c@{}}Accept.\\ Ratio\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Load \\ Balance\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Cost and \\ Revenue\end{tabular} &
  SLA &
  CNN &
  GCN &
  \begin{tabular}[c]{@{}c@{}}Value\\ Based\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Policy\\ Based\end{tabular} &
   \\ \midrule
\cite{p1}                 & \checkmark &   & \checkmark &   & \checkmark & \checkmark & \checkmark &   &   & \checkmark &     & A3C     &   \\ \midrule
\cite{rkhami2021learn} & \checkmark &   & \checkmark &   &   &   & \checkmark &   &   & \checkmark &     & REIN    & \checkmark \\ \midrule
\cite{p2}             & \checkmark &   & \checkmark &   &   &   & \checkmark &   & \checkmark &   & DQL &         &   \\ \midrule
\cite{p3}                & \checkmark & \checkmark & \checkmark & \checkmark &   &   &   & \checkmark & \checkmark &   &     & RMSProp &   \\ \midrule
\cite{p4}                & \checkmark &   & \checkmark & \checkmark & \checkmark &   & \checkmark &   & \checkmark &   &     & PG      &   \\ \midrule
\cite{p5}                & \checkmark &   & \checkmark &   &   &   & \checkmark &   &   &   &     & PG      &   \\ \midrule
\cite{quang2019deep}    & \checkmark &   & \checkmark & \checkmark & \checkmark &   &   &   & \checkmark &   &     & DDPG    & \checkmark \\ \midrule
\cite{p8}               & \checkmark &   & \checkmark & \checkmark &   &   & \checkmark &   & \checkmark &   &     & DDPG    &   \\ \bottomrule
\end{tabular}
\end{table*}

==> Backup/old_HA-DRL_text.tex <==
Algorithm \ref{alg::drl_and_p2c} presents a pseudocode of our procedure to train the DRL agent for Network Slice Placement Optimization using P2C heuristic as external control for A3C (see Sections \ref{sec:problem_statement_and_formulation} and \ref{sec::drl_feamework} for a complete explanation of the notations). To improve the learning results, we allow the DRL agent during the training process to activate the P2C heuristic when its policy selects an a unsuccessful action (i.e., a placement node that does not have enough avaliable resources to receive the current VNF or that cannot be interconnected to the previous ones) as described in lines \ref{line::if_unsuccessful_1}-\ref{line::if_unsuccessful_2}. The heuristic then tries to find another node to place the current VNF and if it succeeds, this action is applied to the environment that calculate the respective reward and the gradients for updating the deep neural networks (lines \ref{line::p2c_finds_better_action_1}-\ref{line::p2c_finds_better_action_2}). Note that here we calculate only $\nabla_{\theta_{v}}V^{\pi_{\theta}}_{\theta_{v}}(S_{t})$ at each time step since we cannot directly calculate $\nabla_{\theta_{v}}A^{\pi_{\theta}}(S_t,a_t)^{2}$ iteratively. 

The procedure stops when it achieves a terminal state, that is when there is a blocking on the placement of the current NSPR or when the placement is complete. We then update the deep neural networks using the rules introduced by Equations (\ref{eq::update_rules_1}) and (\ref{eq::update_rules_2}) based on the results returned by Algorithm \ref{alg::drl_and_p2c}. We obtain the gradient $\nabla_{\theta_{v}}A^{\pi_{\theta}}(S_t,a_t)^{2}$ by applying the chain rule $\nabla_{\theta_{v}}A^{\pi_{\theta}}(S_t,a_t)^{2} =2A^{\pi_{\theta}}(S_t,a_t) ( \nabla_{\theta_{v}}V^{\pi_{\theta}}_{\theta_{v}}(S_{t+1}) - \nabla_{\theta_{v}}V^{\pi_{\theta}}_{\theta_{v}}(S_{t})$).


\begin{algorithm}
%\tiny
%\scriptsize
\SetAlgoLined
 \KwData{$\theta$, $\theta_v$,$G_s$,$S_t$}
 \KwResult{$\Delta^{\theta}, \Delta^{\theta_{v}}$}
  $continue \leftarrow true$ \tcp*{Loop variable}
  $\Delta^{\theta} \leftarrow  \{\}$ \tcp*{Vector of gradients w.r.t. $\theta$}
  $\Delta^{\theta_{v}} \leftarrow  \{\}$ \tcp*{Vector of gradients w.r.t. $\theta_{v}$}
  \While{$continue$}{
        $a_{drl} \leftarrow 0$ \tcp*{Action selected by DRL agent}
        $r_{drl} \leftarrow 0$ \tcp*{Reward due to $a_{drl}$}
        $a_{p2c} \leftarrow 0$ \tcp*{Action selected by P2C heuristic}
        $r_{p2c} \leftarrow -\infty$ \tcp*{Reward due to $a_{p2c}$}
        $r_{drl},a_{drl},V^{\pi_{\theta}}_{\theta_{v}}(S_{t}) \leftarrow$ DRL($\theta, \theta_v,S_t,G_s$)\;
        $status \leftarrow get\_status(a_{drl},S_t)$\;
        \If{$status = $ Unsuccessful}{ \label{line::if_unsuccessful_1}
            $r_{p2c},a_{p2c}, \leftarrow$ P2C($S_t,G_s$) \label{line::if_unsuccessful_2} \;    
        }
        \eIf{$r_{p2c} > r_{drl}$}{ \label{line::p2c_finds_better_action_1}
            $a_{t} \leftarrow a_{p2c}$\;
            $r_{t+1} \leftarrow r_{p2c}$\;
        }{
            $a_{t} \leftarrow a_{drl}$\;
            $r_{t+1} \leftarrow r_{drl}$\;
        }
        $\Delta^{\theta} \leftarrow \Delta^{\theta} \cup \{\nabla_{\theta}log\pi_{\theta}(a_t|S_t)\}$\;
        $\Delta^{\theta_{v}} \leftarrow \Delta^{\theta_{v}} \cup \{\nabla_{\theta_{v}}V^{\pi_{\theta}}_{\theta_{v}}(S_{t})\}$\;
        $S_{t} \leftarrow S_{t+1}$ \tcp*{Move to next state based on action $a_{t}$} \label{line::p2c_finds_better_action_2}
        \If{$S_{t}$ is terminal}{
            $V^{\pi_{\theta}}_{\theta_{v}}(S_{t}) \leftarrow 0$\;
            $continue \leftarrow false$\; 
        }
  }
  \caption{Training the DRL agent for Network Slice Placement Optimization using P2C heuristic as external control}
  \label{alg::drl_and_p2c}
\end{algorithm}

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

